A Technical Look At The Indian Personal Data Protection Bill

The Indian Personal Data Protection Bill 2019 provides a legal framework for protecting personal data. It is modeled after the European Union's General Data Protection Regulation(GDPR). We present a detailed description of the Bill, the differences with GDPR, the challenges and limitations in implementing it. We look at the technical aspects of the bill and suggest ways to address the different clauses of the bill. We mostly explore cryptographic solutions for implementing the bill. There are two broad outcomes of this study. Firstly, we show that better technical understanding of privacy is important to clearly define the clauses of the bill. Secondly, we also show how technical and legal solutions can be used together to enforce the bill.

==> blockchain.tex <==
% Contents in the second and third columns will be auto-wrapped,
% so that the entire table will fit the text width nicely
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}
\begin{table}[htbp]
 \begin{center}
   \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|}
           \hline
           \rowcolor{LightCyan}
				\textbf{S.No.} &  \textbf{Topics} &  \textbf{Required properties} & \textbf{Blockchain properties} & \textbf{References} \\
			\hline 
				1. & Data consent & Proof of consent, modification of consent,removal of consent & Smart contract & \cite{Blitcoin,Ethereum} \\
			\hline 
			 2. & Proof of user's rights(Right to correction, access and deletion) & Proof of correction, access and deletion & Smart contract  & \cite{Blitcoin,Ethereum} \\
			 \hline 
			 3. & Data audit & Data audit when all three party are malicious & Blockchain auditability & \cite{BC36_blockchainPDP,BDA1} \\
			 \hline
			  4. & Privacy preserving, data sharing & Eg. Healthcare data & Privacy and anonymisation of data & \cite{bc4_healthDataSharing,bc4_Medrec} \\
			  \hline 
			  5. & Privacy in data processing & Privacy preservation by limited data disclosure & Data owner owns data, data market & \cite{bc578_matrimonial}\\
			  \hline
			  6. & Access control & Ownership and access of data, prevention from security breaches & Blockchain based access control & \cite{bc6_accessControl,BC36_blockchainPDP,bc8_2_proofOfLocation} \\
			  \hline
			  7. & Data collection & anonymity, limited data collection  & Privacy preserving search using blockchain in data market & \cite{Blitcoin,bc578_matrimonial,bc78_DataMarket} \\
			  \hline
			  8. & Proof of X & Proof of storage, retrievability, proof of data ownership, location & Blockchain based proofs & \cite{bc8_2_proofOfLocation,bc8_3_RetrieCoin,bc8_1_OPOR,bc78_DataMarket,bc578_matrimonial} \\
			  \hline
			  9. & Ownership transfer of personal data & Asset transfer & Smart contract & \cite{Blitcoin,Ethereum} \\
			 \hline
			 10. & Security breaches & Independent from single point of failure, integrity of data and  storage,  & Distributed storage of data, fault tolerance, proof of data, storage, retrievability & \cite{bc10_1_DataStorageIoT,bc10_2_transparency}   \\
			 \hline 
			 11. & Transparency & Transparency in data processing & Trust distribution, public verifiability, auditability, smart contract, immutability  & \cite{Ethereum,bc11_transparency}    \\
		
		   \hline
      \end{tabularx}\caption{Blockchain for data protection }\label{table:blockchain_DP}
	%\begin{tabular}{|l|l|l|l|l|}
	%\end{tabular}
  \end{center}
\end{table}

==> pointsbill.tex <==


\begin{table}[htbp]
		\begin{center}
			
			\begin{tabular}{|l|l|l|}
				\hline
				Data principal consent & Data Collection & Data Processing \\
				\hline
				Privacy by Design and  Transparency & Data breaches &Data audit \\
				\hline 
				Rights of Data principal & Processing of Children's data
				& Localization of \\
				& & sensitive personal data \\
				\hline
				\end{tabular} \caption{Properties need to be taken care while designing a system under Indian Data protection privacy bill }\label{table:pointsbill}
		\end{center}
	\end{table}
